Machine Learning Aided Holistic Handover Optimization for Emerging Networks

In the wake of network densification and multi-band operation in emerging cellular networks, mobility and handover management is becoming a major bottleneck. The problem is further aggravated by the fact that holistic mobility management solutions for different types of handovers, namely inter-frequency and intra-frequency handovers, remain scarce. This paper presents a first mobility management solution that concurrently optimizes inter-frequency related A5 parameters and intra-frequency related A3 parameters. We analyze and optimize five parameters namely A5-time to trigger (TTT), A5-threshold1, A5-threshold2, A3-TTT, and A3-offset to jointly maximize three critical key performance indicators (KPIs): edge user reference signal received power (RSRP), handover success rate (HOSR) and load between frequency bands. In the absence of tractable analytical models due to system level complexity, we leverage machine learning to quantify the KPIs as a function of the mobility parameters. An XGBoost based model has the best performance for edge RSRP and HOSR while random forest outperforms others for load prediction. An analysis of the mobility parameters provides several insights: 1) there exists a strong coupling between A3 and A5 parameters; 2) an optimal set of parameters exists for each KPI; and 3) the optimal parameters vary for different KPIs. We also perform a SHAP based sensitivity to help resolve the parametric conflict between the KPIs. Finally, we formulate a maximization problem, show it is non-convex, and solve it utilizing simulated annealing (SA). Results indicate that ML-based SA-aided solution is more than 14x faster than the brute force approach with a slight loss in optimality.

==> Tables.tex <==
\begin{table}[t]
\centering
\caption{Prediction of Mean RSRP}
\label{table:RSRPpred}
\begin{tabular}{|>{\centering\arraybackslash} m{2cm} | >{\centering\arraybackslash} m{1.5cm}| >{\centering\arraybackslash} m{1cm}| >{\centering\arraybackslash} m{1.5cm}|}
\hline
\textbf{Model} & \textbf{Root Mean Square Error (dBm)} & \textbf{R2 Score} & \textbf{Mean Cross-Validation Score}                \\ \hline
Linear Regression & 0.4613 & 0.6628 & 0.6798                    \\ \hline
Polynomial Regression & 0.1859 & 0.9452 & 0.6798                     \\ \hline
Support Vector Regression & 0.1228 & 0.9761 & 0.9784                    \\ \hline
Decision Tree Regression & 0.0930 & 0.9863 & 0.9859                     \\ \hline
Random Forest Regression & 0.0748 & 0.9911 & 0.9908                     \\ \hline
XGBoost Regression & 0.0737 & 0.9914 & 0.9919                 \\ \hline
\end{tabular}
\end{table}

\subsubsection{RLF Rate}
\begin{table}[t]
\centering
\caption{Prediction of Handover Success Rate}
\label{table:RLFpred}
\begin{tabular}{|>{\centering\arraybackslash} m{2cm} | >{\centering\arraybackslash} m{1.5cm}| >{\centering\arraybackslash} m{1cm}| >{\centering\arraybackslash} m{1.5cm}|}
\hline
\textbf{Model} & \textbf{Root Mean Square Error} & \textbf{R2 Score} & \textbf{Mean Cross-Validation Score}                \\ \hline
Linear Regression & 0.0559 & 0.4471 & 0.4556                    \\ \hline
Polynomial Regression & 0.0474 & 0.6026 & 0.4556                     \\ \hline
Support Vector Regression & 0.0495 & 0.5671 & 0.5610                    \\ \hline
Decision Tree Regression & 0.0337 & 0.7995 & 0.7177                     \\ \hline
Random Forest Regression & 0.0258 & 0.8826 & 0.8223                     \\ \hline
XGBoost Regression & 0.0250 & 0.8893 & 0.8304                 \\ \hline
\end{tabular}
\end{table}
